The Wasserstein Believer: Learning Belief Updates for Partially Observable Environments through Reliable Latent Space Models

Partially Observable Markov Decision Processes (POMDPs) are used to model environments where the full state cannot be perceived by an agent. As such the agent needs to reason taking into account the past observations and actions. However, simply remembering the full history is generally intractable due to the exponential growth in the history space. Maintaining a probability distribution that models the belief over what the true state is can be used as a sufficient statistic of the history, but its computation requires access to the model of the environment and is often intractable. While SOTA algorithms use Recurrent Neural Networks to compress the observation-action history aiming to learn a sufficient statistic, they lack guarantees of success and can lead to sub-optimal policies. To overcome this, we propose the Wasserstein Belief Updater, an RL algorithm that learns a latent model of the POMDP and an approximation of the belief update. Our approach comes with theoretical guarantees on the quality of our approximation ensuring that our outputted beliefs allow for learning the optimal value function.

==> related_work.tex <==


POMDPs pose a significant challenge to RL due to the loss of the Markovian property --- the next observation distribution do not only depend on the current state, but on the entire action-observation history.
As a consequence, this history need be considered to derive an optimal policy, making it essential to obtain a sufficient statistic such as belief states \cite{kaelbling1998planning}. Most deep-RL methods use RNNs to compress the action-observation history into a fixed-size vector \cite{Hausknecht2015DeepMDPs} and apply regularization techniques to improve the likelihood of obtaining a belief. These techniques include generative models \cite{chen2022flow, Hafner2019DreamImagination, hafner2021mastering}, particle filtering \cite{Igl2018DeepPOMDPs, ma2020particle}, and predicting distant observations \cite{Gregor2018TemporalAuto-Encoder, Gregor2019ShapingRL}. 
However, most algorithms assume the beliefs to be simple distributions of states, such as Gaussian distributions, limiting their applicability \cite{Gregor2018TemporalAuto-Encoder, lee2020stochastic, hafner2021mastering}. We note that using Normalizing Flows for the belief distribution as been experienced in FORBES \cite{chen2022flow}. However, FORBES does not condition its policy on the beliefs but rather on sample latent states (which is known to be sub-optimal)\todo{F: ref}.
Some works also focus on specific types of POMDPs, such as building compact latent representation of images for visual motor tasks \cite{lee2020stochastic}, or environment where the observation are masked states with Gaussian noise \cite{wang2021deep}. 
In contrast to those works building on beliefs merely for improving learning, WBU's beliefs are tailored to adhere to the belief update rule of a latent space model, which exhibits behaviors equivalent to those of the environment. This yields a guaranteed, suitable representation for optimizing returns.

While accessing the state is common in partially observable deep multi-agent RL, and known as the centralized training decentralized execution paradigm \cite{Oliehoek2008OptimalPOMDPs, Avalos2022LocalLearning}, it is not a common practice in single-agent RL with the exception of kernel-POMDPs  \cite{Nishiyama2012HilbertPOMDPs} that uses the states to build models based on RKHSs. \todo{maybe insist here about the applicability of accessing the state}

Finally, the works of \cite{DBLP:conf/icml/GeladaKBNB19,aaai-2023-delgrange-nowe-perez} study similar value difference bounds to ours in the context of fully observable environments, guaranteeing the quality of (i) the latent space model learned, and (ii) the representation induced by $\embed_{\encoderparameter}$ for optimizing the returns.
They further link their bounds with bisimulation theory (e.g., \cite{DBLP:conf/popl/LarsenS89,DBLP:journals/ai/GivanDG03}). %
We defer as future work the study of bisimulation metrics \cite{DBLP:journals/tcs/DesharnaisGJP04,DBLP:journals/siamcomp/FernsPP11} in the context of POMDPs.








    

